Active Visuo-Tactile Point Cloud Registration for Accurate Pose Estimation of Objects in an Unknown Workspace

This paper proposes a novel active visuo-tactile based methodology wherein the accurate estimation of the time-invariant SE(3) pose of objects is considered for autonomous robotic manipulators. The robot equipped with tactile sensors on the gripper is guided by a vision estimate to actively explore and localize the objects in the unknown workspace. The robot is capable of reasoning over multiple potential actions, and execute the action to maximize information gain to update the current belief of the object. We formulate the pose estimation process as a linear translation invariant quaternion filter (TIQF) by decoupling the estimation of translation and rotation and formulating the update and measurement model in linear form. We perform pose estimation sequentially on acquired measurements using very sparse point cloud as acquiring each measurement using tactile sensing is time consuming. Furthermore, our proposed method is computationally efficient to perform an exhaustive uncertainty-based active touch selection strategy in real-time without the need for trading information gain with execution time. We evaluated the performance of our approach extensively in simulation and by a robotic system.

==> figures/object_table.tex <==
%\begin{table}[h!]
%%     \begin{center}
%     \begin{tabular}{ | c | c | c | c | c | }
%     \toprule

%     \includegraphics[width=\linewidth]{figures/objects/olive_oil.png}
%      & 
%      \raisebox{.5\height}{\includegraphics[width=0.02\textwidth]{figures/objects/detergent.png}}
%      & 
%      \raisebox{.5\height}{\includegraphics[width=0.02\textwidth]{figures/objects/shampoo.png}}
%      &
%%      \includegraphics[width=0.02\textwidth]{figures/objects/sugar_big.png}
%      &
%      \includegraphics[width=0.02\textwidth]{figures/objects/sugar_big.png}
%      \\ 
%      \hline
%      Object1 & Object2 & Object3 & Object4 & Object5 \\ 
%      \bottomrule
%      \end{tabular}
%%      \caption{Object List}
%      \label{tbl:object_list}
%      \end{center}
%\end{table}

 %\begin{table}[h!]
 %\begin{center}
 %\begin{tabular}{|c|c|c|c|c|c|}
 %\hline
 %Olive Bottle & Shampoo & Detergent & Window Spray & Sugar Box & Can  \\
 %\hline
 %\raisebox{-.5\height}{\includegraphics[scale=0.01]{figures/object_images/Olive.pdf}} & \raisebox{-.5\height}{\includegraphics[scale=0.01]{figures/object_images/shampoo.png}} &  \raisebox{-.5\height}{\includegraphics[scale=0.01]{figures/object_images/detergent.png}} & \raisebox{-.5\height}{\includegraphics[scale=0.01]{figures/object_images/sugar_big.png}} &  \raisebox{-.5\height}{\includegraphics[scale=0.01]{figures/object_images/sugar_big.png}} & \raisebox{-.5\height}{\includegraphics[scale=0.01]{figures/object_images/beans_can.png}} \\

% \hline
% Object1 & Object2 & Object3 & Object4 & Object5 & Object 6 \\ 
% \hline
%\end{tabular}
%\label{Objects used for robot experiments}
%\end{center}
%\end{table}



==> figures/table_correction.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Object} & \multicolumn{2}{c|}{\textbf{Vision}} & \multicolumn{2}{c|}{\textbf{Vision and Tactile}} \\ \hline
                & RMSE Pos (mm)          & RMSE Rot (deg)        & RMSE Pos (mm)                & RMSE Rot (deg) \\ \hline
Glass Bottle    & $8.745354 \pm 3.910463$& $7.99464 \pm 0.989942$&$6.116598 \pm 3.274342$  &$3.816942 \pm 2.316518$  \\ \hline
Plastic Shampoo &$7.9489 \pm 2.9582$  & $8.2130 \pm 2.2323$&$4.536149 \pm 3.044584$  &$4.835901 \pm 2.630103$  \\\hline
Cleaner         &$9.8513 \pm 4.331742956$&$8.5617 \pm 2.01393$ &$6.2469434 \pm  2.92317$ &$4.368895 \pm 1.1873161$ \\ \hline
    Spray       &$11.598367 \pm 4.9172706$ & $9.117646 \pm 2.2031033$&$3.350447 \pm 1.013378$  &$4.591424 \pm 0.9722974$ \\ \hline
    Sugar box   &$12.249184 \pm 5.608618$& $8.624424 \pm 3.097540960094798$&$6.454406 \pm 3.204113$  &$4.134275\pm 1.4037660$ \\ \hline
\end{tabular}}
\end{table*}


==> sections/background.tex <==
\section{BACKGROUND}
\label{sec:background}

% \begin{itemize}
%     \item Definition of notations used in the paper: Formalization of point clouds, dual quaternions and DQF filter.
%     \item Assumptions used in the paper
%     % guarded move: An Experimental System for Computer Controlled mechanical assembly
% \end{itemize}



==> sections/legacy/methods.tex <==
\section{METHODS}
\label{sec:methods}


%-Generative model we want to use
%-Show decoupling of rotation and translation (mention that this can be done without even considering dual-quaternions)
%-Show closed form solution for translation
%-We pose the active object localization problem as a bayesian filtering problem
%-Show short derivation of formula with actions
%-Show that this leads to a Kalman filter
%-We decide to use quaternions as smooth representation, since we need a linear model for the kalman filter

%-Thats why we want to use dual-quaternions
%-Write the generative model as dual-quaternion
%-Looking at two pairs of correspondences we can construct translation invariant measurements
%-Therefore we can decouple translation and rotation
%-Write down the generative model for this 
%-Write down the objective
%-This is linear and we have continuously arriving measurements, also we want to reason over how possible actions affect the result
%-Therefore we will incorporate this into a bayesian filter
%-Bayesian approach to object localization (bayesian network)
%-Write down equations, then write down assumptions
%-Then we get to a Kalman filter
%-To incorporate the above generative model we use matrix formulation of this equation we use the concept of pseudo measurements
%-Derive all equations for kalman
%-This leads us to DQF (parametrized by an action)
%-To perform the action selection we will adopt a scheme known from other works
%-How to parametrize the state vector?
%-

\subsection{Problem Formulation}
\begin{figure*}[bt]
    \centering
    \includegraphics[width = 0.8\textwidth, height = 8cm]{figures/framework.png}
    \caption{Framework for vision based active tactile object localization}
    \label{fig:framework}
\end{figure*}
Given $N$ objects $o_i$ for $i = 1,2,\dots,N$ in the workspace $W_{XYZ}$ of the robot with unknown poses. The workspace $W_{XYZ}$ is defined as a discretised 3D grid bounded by the kinematic reaching constraints of the robot and defined in the world coordinate frame $\mathcal{W}$. Given Assumption~\ref{assumption2:static}, the pose of each object is static in time. Furthermore, given Assumption~\ref{assumption1:cad}, each object $o_i$ has a coordinate frame $\mathcal{O}_i$ rigidly attached to the geometric model of the object. The objective is to find the object pose ${}^{\mathcal{W}} H_{\mathcal{O}_i}$ for $i=1,2,3,\dots ,N$ given external sensor measurements from vision sensor $z^{v}$ and tactile sensor $z_0, z_1, z_2, \dots, z_t$. An initial pose estimate is extracted using the vision sensor measurement at time $t=0$ whereas the estimated pose is \textit{corrected} using sequential measurements from the tactile sensor collected in an \textit{active} manner by the robot.
\todo[inline]{Math-Cal symbols don't look good}
\todo[inline]{Definition of vision sensor and tactile sensor}
%\subsubsection*{Assumptions}
The assumptions used in this paper is detailed as follows:
\begin{assumption}
\label{assumption1:cad}
We assume that the objects are rigid and we have the geometric model of each object.
\end{assumption}

\begin{assumption}
\label{assumption2:static}
We assume the objects are rigidly attached to the workspace and the object pose does not change during acquiring measurements.
\end{assumption}

\subsection{Vision-Based Pose Estimation}
As described in the framework, the vision-based pose estimation is used for providing a good initial estimate for the pose estimation by active tactile exploration. 
A point cloud $\mathcal{P}$ is acquired by the sensing device, henceforth termed \textit{scene} and is encoded as $ p_i = \{x_i, y_i, z_i \}$ for $p_i \in \mathcal{P}$ described in the frame of the sensing device $S$. The point cloud $\mathcal{P}$ is transformed to a global world frame $W$ by applying the known ${}^{W} H_{S}$ homogeneous transformation. In order to simplify the process of object localisation, it is common to perform pre-processing steps in order to remove points of non-interest from $\mathcal{P}$. Making use of contextual knowledge of the scene wherein the object are placed on a supporting planar structure, the vision algorithm performs plane segmentation in order to search and remove the plane. 
Random sample consensus (RANSAC)~\cite{fischler1981random} is used to generate model hypothesis in order to extract the inlier points for the best fitting plane. For the inlier points, we employ a least squares approach to estimate the model coefficients for the plane and the points satisfying the plane equation with a user specified tolerance is removed. The remaining points are \textit{clustered} based on the L2 norm between points to provide $\kappa$ clusters~\cite{rusu2013semantic}. 
We choose the \textit{correspondence-based} point cloud registration paradigm as opposed to iterative closest point (ICP) ~\cite{besl1992method} and related simultaneous correspondence and pose methods (\textit{correspondence-free}) due to the presence of multiple objects in the scene and lack of good initial guess to guide ICP. 
In the correspondence-based setup, the problem of point cloud registration is formalised as follows: given two point clouds $\mathcal{A} = \{\mathbf{a_i}\}_{i=1}^{N}$ and $\mathcal{B} = \{\mathbf{b_i}\}_{i=1}^{N}$ with $\mathbf{a_i}, \mathbf{b_i} \in \mathbb{R}^3$ that obey the following generative model:
\begin{equation}
    \mathbf{a_i} = \mathbf{R}\mathbf{b_i} + \mathbf{t} \quad i = 1,2, \dots N,
    \label{eq:generativemodel}
\end{equation}
where $\mathbf{R} \in SO(3)$ and $\mathbf{t} \in \mathbb{R}^3$ are unknown and need to be computed and Equation~\eqref{eq:generativemodel} assumes no scale and measurement noise.
In generic applications involving object localisation, $\mathbf{a_i}$ are points belonging to the scene and $\mathbf{b_i}$ are points from the CAD model of the object.
In our approach, we extract putative correspondences using Fast Point Feature Histograms (FPFH)~\cite{rusu2009fast}. The 
registration step is performed using RANSAC. Furthermore, in order to evaluate the robustness of the pipeline, we also perform the registration with the state-of-art certifiably robust algorithm termed TEASER++~\cite{yang2020teaser}. The output of the vision estimate is provided as \textit{initial belief} for the tactile localisation computation.

\subsection{Tactile-Based Pose Estimation}
First we decouple rotation and translation estimation similarly to previous work. We then formulate the rotation estimation problem in a Bayesian manner. Finally, we formulate assumptions and arrive at a linear filter. This allows for very fast computations of candidate states during the action selection.

\subsubsection{Decoupling rotation and translation}
Considering the point cloud registration problem, given known correspondences, we use the generative model as defined in Equation~\eqref{eq:generativemodel}. We adopt a key insight to decouple translation and rotation measurements, without using dual quaternions, as done in prior work~\cite{yang2020teaser, horn1987closed, srivatsan2016estimating}. Given a pair of measurements $\mathbf{a_i}, \mathbf{a_j}$ and their correspondences $\mathbf{b_i}, \mathbf{b_j}$, from Equation~\eqref{eq:generativemodel} we have:
\begin{align}
    \mathbf{a_j} - \mathbf{a_i} &= (\mathbf{R}\mathbf{b_j} + \mathbf{t}) - (\mathbf{R}\mathbf{b_i} + \mathbf{t}) \\
    \mathbf{a}_{ji} &= \mathbf{R}\mathbf{b}_{ji}  \quad . 
    \label{eq:trans_invariance}
\end{align}
Therefore, we can obtain \textit{translation invariant measurements} by defining $\mathbf{a}_{ji} = \mathbf{a}_{j} - \mathbf{a}_{i}$ and $\mathbf{b}_{ji} = \mathbf{b}_{j} - \mathbf{b}_{i}$. Once rotation $\hat{\mathbf{R}}$ is estimated, the translation $\hat{\mathbf{t}}$ can be obtained in closed form by plugging $\hat{\mathbf{R}}$ in Equation \eqref{eq:generativemodel} and solving for $\mathbf{t}$. In practice one would take the mean over a set of correspondences, since makes the resulting translation less susceptible to outliers in the correspondences. 
%\begin{equation}
%    \mathbf{t} = \frac{\mathbf{a}_{j}+ \mathbf{a_{i}}}{2} - \mathbf{R} \frac{\mathbf{b_{j}}+ \mathbf{b_{i}}}{2} \quad .
%    \label{eq:trans_output}
%\end{equation}


%\todo[inline]{Work-in-progress from this point onwards}

\subsubsection{Bayes Filter}

\begin{figure}[bt]
    \centering
    \includegraphics[width = \columnwidth]{figures/bayesian_network.png}
    \caption{Bayesian Networks with standard \textit{Kalman Filter} (left) and our model (right)}
    \label{fig:bayesian_network}
\end{figure}

%We design the problem of localization as a state estimation framework based on a \textit{Bayes Filter}. 
We seek to estimate the rotation object $o_i$. This rotation is defined as the state $\mathbf{x}$ in the latter. According to assumption \ref{assumption2:static} the true state $\mathbf{x}$ is static. To get a better estimate of the state we perform actions $a_t$ with the robot and receive measurements $z_t$, based on the action we chose. This is summarized in a Bayesian network in figure \ref{fig:bayesian_network}. Lets for now not look at how we actually choose $a_t$. 

% \subsubsection{Point Cloud Registration}
% For the general problem of object localization with tactile measurements we stick to the general formalization of point cloud registration with known correspondences.
% \begin{equation}
%     \mathbf{s}_i = \mathbf{R}\mathbf{o}_i + \mathbf{t}
%     \label{eq:gen_model}
% \end{equation}
% $\mathbf{s}_i$ is a point from the scene, i.e. a tactile measurement, and $\mathbf{o}_i$ is a point from the model point cloud. Therefore a correspondence is given by a tuple $(\mathbf{s}_i, \mathbf{o}_i)$. We seek to estimate the global rotation $\mathbf{R}\in SO(3)$ and the global translation $\mathbf{t}\in \mathbb{R}^3$. Like previous works on point cloud registration have already shown, you can decouple the optimization objective by taking pairs of correspondences into consideration. We define vectors between such a pair as $\mathbf{s_{ij}} = \mathbf{s}_j - \mathbf{s}_i$ and $\mathbf{o_{ij}} = \mathbf{o}_j - \mathbf{o}_i$ respectively. Also we know that the same generative model also applies for the defined measures $(\mathbf{s}_{ij}, \mathbf{o}_{ij})$. Therefore we plug this into \eqref{eq:gen_model}:

% \begin{align*}
%     % \mathbf{s}_{ij} &= \mathbf{R}\mathbf{o}_{ij} + \mathbf{t} \\
%     \mathbf{s}_i &= \mathbf{R}\mathbf{o}_i + \mathbf{t} \quad , \\
%     \mathbf{s}_j &= \mathbf{R}\mathbf{o}_j + \mathbf{t} \quad ,\\ 
%     \mathbf{s}_{ij} &= \mathbf{s}_j - \mathbf{s}_i = \mathbf{R}\mathbf{o}_j + \mathbf{t} - \mathbf{R}\mathbf{o}_i + \mathbf{t} = 
%     \mathbf{R} (\mathbf{o}_j - \mathbf{o}_i) \quad ,
% \end{align*}
% \begin{equation}
%     \mathbf{s}_{ij}  = \mathbf{R}\mathbf{o}_{ij} \quad .
%     \label{eq:gen_model_rot}
% \end{equation}
% From equation \ref{eq:gen_model_rot} we can clearly see, that the translation canceled and we can estimate the rotation separately from the translation. After estimating the rotation we can obtain the translation with one given correspondence and the rotation estimate $\hat{\mathbf{R}}$: 
% \begin{align}
%     \mathbf{s}_i &= \hat{\mathbf{R}}\mathbf{o}_i + \mathbf{t} \\
%     \mathbf{t} &= \mathbf{s}_i - \hat{\mathbf{R}}\mathbf{o}_i
% \end{align}
% To get a more stable solution in the end we can also take the mean over all translation estimates given by all correspondences. 

%\subsubsection{Bayesian Filter for static object localization}
%\todo[inline]{Say somewhere, that the measurements here will be correspondences, so define zt. Then we will have it easier when deriving the quaternion formulation}
% As shown in the previous section, we can decouple rotation and translation. Inspired from previous work we will show the derivation of a \textit{Kalman Filter} to estimate the rotation that incorporates actions, such that we can select actions based on their effect on the estimate. As shown in figure \ref{fig:bayesian_network} we consider the object localization problem as a \textit{Markov Chain}. Starting from a bayesian formulation we get to the Kalman equations. 

\begin{align}
    p(\mathbf{x}_t | \mathbf{z}_{1:t}, \mathbf{a}_{1:t}) &= \eta p(\mathbf{x}_t, \mathbf{z}_{1:t},\mathbf{a}_{1:t}) \\
    &= \eta p(\mathbf{z}_{t} | \mathbf{z}_{1:t-1}, \mathbf{x}_t, \mathbf{a}_{1:t}) p(\mathbf{x}_{t-1}, \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t-1}) 
    \label{eq:bayesian_filter:1}
\end{align}
$\eta$ is a normalization constant.Since we assume that the measurements $\mathbf{z}_t$ only depend on the state $\mathbf{x}$ and the action $\mathbf{a}_t$ at timestep $t$, we simplify eq. \ref{eq:bayesian_filter:1}. $(\mathbf{z}_{1:t-1}, \mathbf{a}_{1:t})$ is added into the normalization constant. 
\begin{align}
    p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t}) &= \eta p(\mathbf{z}_{t} | \mathbf{x}, \mathbf{a}_{t}) p(\mathbf{x}, \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t}) \\
    &= \eta p(\mathbf{z}_{t} | \mathbf{x}, \mathbf{a}_{t}) p(\mathbf{x}| \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t-1}) 
    \label{eq:bayesian_filter:2}
\end{align}
% Also we consumed the expression $p(\mathbf{z}_{1:t-1}, \mathbf{a}_{1:t})$ into the normalization constant. 
Note that $p(\mathbf{x}| \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t}) = p(\mathbf{x}| \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t-1})$, since we do not consider the state depending on future actions. 
%\todo[inline]{Dependence on actions is not super clear. Make this simplification more clear}
With equation \ref{eq:bayesian_filter:2}, we arrive at the formalization for object localization in the static case conditioned on the actions. 
\begin{equation}
    bel(\mathbf{x})_t = \eta p(\mathbf{z}_{t} | \mathbf{x}, \mathbf{a}_{t}) bel(\mathbf{x})_{t-1}
    \label{eq:bayesian_kalman}
\end{equation}
Note that, the dependence of $\mathbf{x}$ on the actions is solemnly stemming from the measurement model $p(\mathbf{z}_{t} | \mathbf{x}, \mathbf{a}_{t})$. Since we consider $\mathbf{a}_{t}$ not as a random variable, but as a parameter that is chosen at timestep $t$.
 
% Our goal is to arrive at a linear filter, since this has nice implications on convergence speed and computational complexity. As in previous works we adopt a quaternion formulation for the rotation $\mathbf{x}_t$. Also, w.l.o.g. we assume that $\mathbf{x}$ and $\mathbf{z}_t$ are Gaussian distributed. The action $\mathbf{a}_t$ is chosen at timestep $t$ and is not a random variable, therefore the distribution over the state for the next timestep $p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t})$ will also be Gaussian. We will compare the standard Kalman Filter with our filter to justify the adjustments we make. The bayesian formulation for a standard Kalman Filter is given by: 
% \begin{align}
%     &p(\mathbf{x}_t | \mathbf{z}_{1:t}, \mathbf{u}_{1:t}) =  \\
%     &\eta p(\mathbf{z}_{t} | \mathbf{x}_t) \int p(\mathbf{x}_t | \mathbf{x}_{t-1} \mathbf{u}_{t}) p(\mathbf{x}_{t-1} | \mathbf{z}_{1:t-1}, \mathbf{u}_{1:t-1}) \, d \mathbf{x}_{t-1}
%     \label{eq:standard_kalman}
% \end{align}
% %\todo[inline]{Check technical terms of kalman filter with existing works}
% Comparing this to equation \ref{eq:bayesian_filter:2} we can see that in our case we have an equivalent formulation, if we assume a static process model for the state update and if we remove the control input $\mathbf{u}_{t}$ from the equation. In a standard Kalman Filter the hypothesis is that the state evolves according to the following equation: 
% \begin{equation}
%     \mathbf{x}_t = \mathbf{A}_t \mathbf{x}_{t-1} + \mathbf{B} \mathbf{u}_{t} + \epsilon_t
% \end{equation}
% This is used to for the belief, which is the integral part of equation \ref{eq:standard_kalman}. Given a state the expected measurement is given by: 
% \begin{equation}
%     \mathbf{z}_t = \mathbf{C}_t \mathbf{x}_{t} + \delta_t
% \end{equation}
% First we adapt the state equation. We drop the dependence on $\mathbf{u}_{1:t}$. Also, we inspect equation \ref{eq:bayesian_filter:2} and remember, that in our case the objects are rigidly fixed, so we set $\mathbf{A} = \mathbb{I}_3$. As mentioned above our measurements are correspondence pairs. We start deriving the measurement matrix by setting $\mathbf{z}_t = \mathbf{s}_{ij}$, so our measurement model $\mathbf{C_t}$ maps from the quaternion $\mathbf{x}_t$ to a point pair in the scene $\mathbf{s}_{ij}$ given a corresponding point pair on the object $\mathbf{o}_{ij}$. 
% We start by reformulating equation \ref{eq:gen_model_rot} with quaternions using the quaternion product:
% \begin{equation}
%     \mathbf{s}_{ij} = \widetilde{\mathbf{q}} \cdot \mathbf{o}_{ij} \cdot \widetilde{\mathbf{q}}^*
% \end{equation}
% We showed above how to formulate the quaternion product as a vector-matrix multiplication. Using this we get to: 
% \begin{align}
%     \mathbf{z}_t = \mathbf{s}_{ij} &= F_1(\widetilde{\mathbf{x}}) \cdot F_2(\widetilde{\mathbf{x}^*}) \cdot  \widetilde{\mathbf{o}}_{ij} \\
%     F(\widetilde{\mathbf{x}}) &= \begin{bmatrix}
%                                     x_0 & -\mathbf{x}^T \\
%                                      \mathbf{x} & -\mathbf{x}^{\times} + x_0 \mathbb{I}_3
%                                     \end{bmatrix} \\
%     F_2(\widetilde{\mathbf{x}^*}) &= \begin{bmatrix}
%                                     x_0 & \mathbf{x}^T \\
%                                     - \mathbf{x} & - \mathbf{x}^\times + x_0 \mathbb{I}_3 
%                                     \end{bmatrix} \\
%     \mathbf{z}_t &= \begin{bmatrix}
%                     x_0^2 + \mathbf{x}^T \mathbf{x} & x_0\mathbf{x}^T - \mathbf{x}^T (\mathbf{x}^{\times} + x_0 \mathbb{I}_3) \\
%                     x_0 \mathbf{x} + (\mathbf{x}^{\times} + x_0 \mathbb{I}_3) (-\mathbf{x}) & \mathbf{x} \mathbf{x}^T + (\mathbf{x}^{\times} + x_0 \mathbb{I}_3) \cdot (\mathbf{x}^{\times} + x_0 \mathbb{I}_3)
%                     \end{bmatrix}
%                     \label{eq:quaternion_matrix}
% \end{align}
%\todo[inline]{Above equations are irrelevant. What I want to show is that first we formulate it in a way where zt is equal to a translation invariant measurement. For this we need to formulate the equation such that Ct contains oij and that x is the quaternion}

%\subsubsection{Kalman Filter Equations}
We assume that $\mathbf{x}$ and $\mathbf{z}_t$ are Gaussian distributed. Therefore, \ref{eq:bayesian_kalman} corresponds to a \textit{Kalman Filter} with static process model. To incorporate the translation invariant measurements, as introduced in \eqref{eq:trans_invariance}, we follow the work of \cite{srivatsan2016estimating}. We simply rearrange \eqref{eq:trans_invariance} to 
\begin{equation}
    \hat{\mathbf{a}_{ji}} - \mathbf{q} \odot \hat{\mathbf{b}_{ji}} \odot \mathbf{q}^{-1} = \mathbf{0} 
    \label{eq:quat_objective}
\end{equation}
by substituting with quaternions. Rewriting in matrix form as shown in \textit{Appendix} gives 
\begin{equation}
    \begin{bmatrix}
        0 & -(\mathbf{a}_{ji} - \mathbf{b}_{ij})^T \\
        (\mathbf{a}_{ji} + \mathbf{b}_{ji}) & (\mathbf{a}_j + \mathbf{a}_i + \mathbf{b}_j + \mathbf{b}_i)^{\times}
        \end{bmatrix} \hat{\mathbf{q}} = \mathbf{0} \quad .
        \label{eq:expected_measurement}
\end{equation}
One could optimize \eqref{eq:quat_objective} directly. However, as shown in previous works we can introduce pseudo-measurements in the \textit{Kalman Filter}. This means setting the true measurement always to $\mathbf{z}_t = 0$ and defining the expected measurement as \eqref{eq:expected_measurement}. Considering that we do not have a prediction step, since our process model is static, we can formulate the Kalman equations as

% \todo[inline]{Work-in-progress}
\begin{align}
    \mathbf{x}_{t|t} &= \mathbf{x}_{t-1|t-1} - \mathbf{K}_t \left( \mathbf{H}_t \mathbf{x}_{t-1|t-1} \right) \\
    \Sigma^{\mathbf{x}}_t &= \left( \mathbf{I} - \mathbf{K}_t \mathbf{H}_t \right) \Sigma_{t-1|t-1} \\
    \mathbf{K}_t &= \Sigma^\mathbf{x}_{t-1|t-1} \mathbf{H}^T \left( \mathbf{H}\Sigma^\mathbf{x}_{t-1|t-1} + \Sigma_t^{\mathbf{h}}\right)
\end{align}

\todo[inline]{Mention that we are doing this in a batch fashion}
%\subsubsection{Pseudo measurements}
% To simplify the computations above and make use of pseudo measurements. Therefore we rewrite equation \ref{eq:quaternion_matrix} into the following form:

%\todo[inline]{Make this dependant on the action notation wise}
 
 
 
%\subsubsection{Uncertainties}

%===========================================================================

\subsection{Active Tactile Exploration}
To reduce the number of touches needed to converge to the true position of the object, we need base the action selection on our previous estimate. As shown above we formulated a measurement model for the Kalman Filter, that depends on some action $\mathbf{a}_t$ that is chosen at timestep $t$. The set of all possible actions $\mathcal{A}(\mathbf{\mu}_t)$ depends on the current state-estimate $\mathbf{\mu}_t$. We want to select the action, $\mathbf{a}_t \in \mathcal{A}(\mathbf{\mu}_t)$, that maximizes the information gain. To measure the information gain we use the KL divergence between $p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t})$ and $p(\mathbf{x} | \mathbf{z}_{1:t+1}, \mathbf{a}_{1:t+1}$. However, to get the true $p(\mathbf{x} | \mathbf{z}_{1:t+1}, \mathbf{a}_{1:t+1}$ we would have to perform the action $\mathbf{a}_{t+1}$. Since this is very time-consuming in the real world because of robot motions, we approximate this distribution by using simulation. We choose a set of random actions from $\mathcal{A}(\mathbf{\mu}_t)$, obtain measurements $\hat{\mathbf{z}_{t+1}}$ from the simulation and then compute the resulting update of the distribution. This is repeated for $N_a$ samples. The chosen action $\mathbf{a}_{t+1}$ is then given by
\begin{align}
    &\mathbf{a}_{t+1} = \argmax_{\hat{\mathbf{a}}_{t+1} \in \mathcal{A}(\mathbf{\mu}_t)} KL(p(\mathbf{x} | \hat{\mathbf{z}}_{1:t+1},  \hat{\mathbf{a}}_{1:t+1}) || p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t})) \\
    &= \argmax_{\hat{\mathbf{a}}_{t+1} \in \mathcal{A}} \int_{x} p(\mathbf{x} | \hat{\mathbf{z}}_{1:t+1},  \hat{\mathbf{a}}_{1:t+1}) \log\frac{p(\mathbf{x} | \hat{\mathbf{z}}_{1:t+1},  \hat{\mathbf{a}}_{1:t+1})}{p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t})}dx \quad .
\end{align}
Since both distributions are gaussian, we can solve the above equation in closed form with
\begin{align}
    &\mathbf{a}_{t+1} = \argmax_{\hat{\mathbf{a}}_{t+1} \in \mathcal{A}} \frac{1}{2} \left[ \frac{|\Sigma_t|}{|\hat{\Sigma}_{t+1}|} -k + \right. \\
    &\left. (\hat{\mathbf{\mu}}_{t+1} - \mathbf{\mu}_{t})^T \Sigma_{t}^{-1} (\hat{\mathbf{\mu}}_{t+1} - \mathbf{\mu}_{t}) + Tr(\Sigma_{t}^{-1} \hat{\Sigma}_{t+1}) \vphantom{\frac{|\Sigma_t|}{|\hat{\Sigma}_{t+1}|}} \right]
\end{align}
% \todo[inline]{Define what k is in the equation above}

\subsubsection{Action Selection}
The relative entropy of the state belief at time $t$ is the Kullback-Leibler divergence of the posterior belief $bel(x_{t+1})$ and the prior belief $bel(x_t)$:
\begin{equation}
    IG = \int_{x} bel(x_{t+1})log\frac{bel(x_{t+1})}{bel(x_t)}dx \quad ,
\end{equation}
wherein, $IG$ measures the \textit{Information Gain} by performing a certain action. In the context of the \textit{best next touch} selection, we aim to find the action that \textit{maximises} the highest expected information gain. 
% \begin{itemize}
%     \item hypothetical measurement using future actions.
%     \item ray-mesh intersection for contact point estimation
% \end{itemize}

% \subsubsection{Termination Criteria}
% \begin{itemize}
%     \item Transformation epsilon between iterations
% \end{itemize}

\begin{algorithm}[h]
\SetAlgoLined
\KwResult{$\mathbf{q}$, $\mathbf{t}$, $\Sigma^{q}$}
\textbf{Input: }{$\mathbf{q_0}$, $\mathbf{t_0}$, $\epsilon_q$, $\epsilon_t$, $\mathbf{q_{gt}}$, $\mathbf{t_{gt}}$} \\ 
\textbf{Initialisation:} \\
Measurements point cloud $\mathcal{Z}$ = \{\} \\
Model point cloud $\mathcal{M}$ = $\mathcal{M}_{CAD}$ \\ 
Correspondences $\mathcal{C}$ = \{\} \\
Transform $\mathcal{M}$ to $q_0, t_0$ \\
Estimated Pose $\mathbf{\hat{q}}, \mathbf{t} \leftarrow \mathrm{MAX\_VALUE}$ \\
Initial Error $\Delta \mathbf{q} = abs(Eul(\mathbf{\hat{q}}) - Eul(\mathbf{q}))$, $\Delta \mathbf{t} = abs(Eul(\mathbf{\hat{q}}) - Eul(\mathbf{q}))$ \\ 
\While{$\Delta \mathbf{q} > \epsilon_q$ \&\& $\Delta \mathbf{t} > \epsilon_t$}{
    
    min, max $\leftarrow$ create\_bounding\_box($\mathcal{M}$) \;
    \eIf{size($\mathcal{Z}$) $\leq$ 2}{
        $\mathbf{a}$ = select\_random\_action($\mathbf{q}$, $\mathbf{t}$, $\mathcal{M}$) \\ 
    }
    {
        $a_i$, $\hat{z}_i$ = generate\_actions($\mathbf{q}$, $\mathbf{t}$, $\mathcal{M}$) \\
        Kullback–Leibler divergence $D_{KL}$ = \{\} \\
        \For{i=1 to size($a_i$)}{
            $\hat{\mathcal{S}}$ = $\mathcal{S} \cup \{ \}$ \;
            $\hat{\mathcal{C}}$ = est\_correspondences($\mathbf{q}$, $\mathbf{t}$, $\mathcal{M}$, $\hat{\mathcal{S}}$) \;
            $\hat{\mathbf{q}}$, $\hat{\Sigma}^q$, $\hat{\mathbf{t}}$ = tiq\_filter.update($\mathbf{q}$, $\Sigma^q$, $\hat{\mathcal{C}}$) \;
            KL.append(compute\_kl\_div($\hat{\mathbf{q}}$, $\hat{\Sigma}^q$, $\mathbf{q}$, $\Sigma^q$) \;
            
        $\mathbf{a}$ = $a_L$[argmax(KL)] \;
        }
     }
}   
\caption{Active tactile exploration for object localisation}
\end{algorithm}







%-----------------------------------------Before making it shorter-----------------------------------------------------------

\section{METHODS}
\label{sec:methods}


%-Generative model we want to use
%-Show decoupling of rotation and translation (mention that this can be done without even considering dual-quaternions)
%-Show closed form solution for translation
%-We pose the active object localization problem as a bayesian filtering problem
%-Show short derivation of formula with actions
%-Show that this leads to a Kalman filter
%-We decide to use quaternions as smooth representation, since we need a linear model for the kalman filter

%-Thats why we want to use dual-quaternions
%-Write the generative model as dual-quaternion
%-Looking at two pairs of correspondences we can construct translation invariant measurements
%-Therefore we can decouple translation and rotation
%-Write down the generative model for this 
%-Write down the objective
%-This is linear and we have continuously arriving measurements, also we want to reason over how possible actions affect the result
%-Therefore we will incorporate this into a bayesian filter
%-Bayesian approach to object localization (bayesian network)
%-Write down equations, then write down assumptions
%-Then we get to a Kalman filter
%-To incorporate the above generative model we use matrix formulation of this equation we use the concept of pseudo measurements
%-Derive all equations for kalman
%-This leads us to DQF (parametrized by an action)
%-To perform the action selection we will adopt a scheme known from other works
%-How to parametrize the state vector?
%-

\subsection{Problem Formulation}
\begin{figure*}[bt]
    \centering
    \includegraphics[width = 0.8\textwidth, height = 8cm]{figures/framework.png}
    \caption{Framework for vision based active tactile object localization}
    \label{fig:framework}
\end{figure*}
Given $N$ objects $o_i$ for $i = 1,2,\dots,N$ in the workspace $W_{XYZ}$ of the robot with unknown poses. The workspace $W_{XYZ}$ is defined as a discretised 3D grid bounded by the kinematic reaching constraints of the robot and defined in the world coordinate frame $\mathcal{W}$. Given Assumption~\ref{assumption2:static}, the pose of each object is static in time. Furthermore, given Assumption~\ref{assumption1:cad}, each object $o_i$ has a coordinate frame $\mathcal{O}_i$ rigidly attached to the geometric model of the object. The objective is to find the object pose ${}^{\mathcal{W}} H_{\mathcal{O}_i}$ for $i=1,2,3,\dots ,N$ given external sensor measurements from vision sensor $z^{v}$ and tactile sensor $z_0, z_1, z_2, \dots, z_t$. An initial pose estimate is extracted using the vision sensor measurement at time $t=0$ whereas the estimated pose is \textit{corrected} using sequential measurements from the tactile sensor collected in an \textit{active} manner by the robot.
\todo[inline]{Math-Cal symbols don't look good}
\todo[inline]{Definition of vision sensor and tactile sensor}
%\subsubsection*{Assumptions}
The assumptions used in this paper is detailed as follows:
\begin{assumption}
\label{assumption1:cad}
We assume that the objects are rigid and we have the geometric model of each object.
\end{assumption}

\begin{assumption}
\label{assumption2:static}
We assume the objects are rigidly attached to the workspace and the object pose does not change during acquiring measurements.
\end{assumption}

\subsection{Vision-Based Pose Estimation}
As described in the framework, the vision-based pose estimation is used for providing a good initial estimate for the pose estimation by active tactile exploration. 
A point cloud $\mathcal{P}$ is acquired by the sensing device, henceforth termed \textit{scene} and is encoded as $ p_i = \{x_i, y_i, z_i \}$ for $p_i \in \mathcal{P}$ described in the frame of the sensing device $S$. The point cloud $\mathcal{P}$ is transformed to a global world frame $W$ by applying the known ${}^{W} H_{S}$ homogeneous transformation. In order to simplify the process of object localisation, it is common to perform pre-processing steps in order to remove points of non-interest from $\mathcal{P}$. Making use of contextual knowledge of the scene wherein the object are placed on a supporting planar structure, the vision algorithm performs plane segmentation in order to search and remove the plane. 
Random sample consensus (RANSAC)~\cite{fischler1981random} is used to generate model hypothesis in order to extract the inlier points for the best fitting plane. For the inlier points, we employ a least squares approach to estimate the model coefficients for the plane and the points satisfying the plane equation with a user specified tolerance is removed. The remaining points are \textit{clustered} based on the L2 norm between points to provide $\kappa$ clusters~\cite{rusu2013semantic}. 
We choose the \textit{correspondence-based} point cloud registration paradigm as opposed to iterative closest point (ICP) ~\cite{besl1992method} and related simultaneous correspondence and pose methods (\textit{correspondence-free}) due to the presence of multiple objects in the scene and lack of good initial guess to guide ICP. 
In the correspondence-based setup, the problem of point cloud registration is formalised as follows: given two point clouds $\mathcal{A} = \{\mathbf{a_i}\}_{i=1}^{N}$ and $\mathcal{B} = \{\mathbf{b_i}\}_{i=1}^{N}$ with $\mathbf{a_i}, \mathbf{b_i} \in \mathbb{R}^3$ that obey the following generative model:
\begin{equation}
    \mathbf{a_i} = \mathbf{R}\mathbf{b_i} + \mathbf{t} \quad i = 1,2, \dots N,
    \label{eq:generativemodel}
\end{equation}
where $\mathbf{R} \in SO(3)$ and $\mathbf{t} \in \mathbb{R}^3$ are unknown and need to be computed and Equation~\eqref{eq:generativemodel} assumes no scale and measurement noise.
In generic applications involving object localisation, $\mathbf{a_i}$ are points belonging to the scene and $\mathbf{b_i}$ are points from the CAD model of the object.
In our approach, we extract putative correspondences using Fast Point Feature Histograms (FPFH)~\cite{rusu2009fast}. The 
registration step is performed using RANSAC. Furthermore, in order to evaluate the robustness of the pipeline, we also perform the registration with the state-of-art certifiably robust algorithm termed TEASER++~\cite{yang2020teaser}. The output of the vision estimate is provided as \textit{initial belief} for the tactile localisation computation.

\subsection{Tactile-Based Pose Estimation}
First we decouple rotation and translation estimation similarly to previous work. We then formulate the rotation estimation problem in a Bayesian manner. Finally, we formulate assumptions and arrive at a linear filter. This allows for very fast computations of candidate states during the action selection.

\subsubsection{Decoupling rotation and translation}
Considering the point cloud registration problem, given known correspondences, we use the generative model as defined in Equation~\eqref{eq:generativemodel}. We adopt a key insight to decouple translation and rotation measurements, without using dual quaternions, as done in prior work~\cite{yang2020teaser, horn1987closed, srivatsan2016estimating}. Given a pair of measurements $\mathbf{a_i}, \mathbf{a_j}$ and their correspondences $\mathbf{b_i}, \mathbf{b_j}$, from Equation~\eqref{eq:generativemodel} we have:
\begin{align}
    \mathbf{a_j} - \mathbf{a_i} &= (\mathbf{R}\mathbf{b_j} + \mathbf{t}) - (\mathbf{R}\mathbf{b_i} + \mathbf{t}) \\
    \mathbf{a}_{ji} &= \mathbf{R}\mathbf{b}_{ji}  \quad . 
    \label{eq:trans_invariance}
\end{align}
Therefore, we can obtain \textit{translation invariant measurements} by defining $\mathbf{a}_{ji} = \mathbf{a}_{j} - \mathbf{a}_{i}$ and $\mathbf{b}_{ji} = \mathbf{b}_{j} - \mathbf{b}_{i}$. Once rotation $\hat{\mathbf{R}}$ is estimated, the translation $\hat{\mathbf{t}}$ can be obtained in closed form by plugging $\hat{\mathbf{R}}$ in Equation \eqref{eq:generativemodel} and solving for $\mathbf{t}$. In practice one would take the mean over a set of correspondences, since makes the resulting translation less susceptible to outliers in the correspondences. 
%\begin{equation}
%    \mathbf{t} = \frac{\mathbf{a}_{j}+ \mathbf{a_{i}}}{2} - \mathbf{R} \frac{\mathbf{b_{j}}+ \mathbf{b_{i}}}{2} \quad .
%    \label{eq:trans_output}
%\end{equation}


%\todo[inline]{Work-in-progress from this point onwards}

\subsubsection{Bayes Filter}

\begin{figure}[bt]
    \centering
    \includegraphics[width = \columnwidth]{figures/bayesian_network.png}
    \caption{Bayesian Networks with standard \textit{Kalman Filter} (left) and our model (right)}
    \label{fig:bayesian_network}
\end{figure}

%We design the problem of localization as a state estimation framework based on a \textit{Bayes Filter}. 
We seek to estimate the rotation object $o_i$. This rotation is defined as the state $\mathbf{x}$ in the latter. According to assumption \ref{assumption2:static} the true state $\mathbf{x}$ is static. To get a better estimate of the state we perform actions $a_t$ with the robot and receive measurements $z_t$, based on the action we chose. This is summarized in a Bayesian network in figure \ref{fig:bayesian_network}. Lets for now not look at how we actually choose $a_t$. Formalizing this we get 
\begin{align}
    p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t}) &= \eta p(\mathbf{x}, \mathbf{z}_{1:t},\mathbf{a}_{1:t}) \\
    &= \eta p(\mathbf{z}_{t} | \mathbf{x}, \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t}) p(\mathbf{x}, \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t}) \quad ,
    \label{eq:bayesian_filter:1}
\end{align}
where $\eta$ is a normalization constant. We assume that the measurements $\mathbf{z}_t$ only depend on the state $\mathbf{x}$ and the action $\mathbf{a}_t$ at timestep $t$. With this we simplify Equation \ref{eq:bayesian_filter:1} and add $p(\mathbf{z}_{1:t-1}, \mathbf{a}_{1:t})$ to the normalization constant. 
\begin{align}
    p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t}) &= \eta p(\mathbf{z}_{t} | \mathbf{x}, \mathbf{a}_{t}) p(\mathbf{x}, \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t}) \\
    &= \eta p(\mathbf{z}_{t} | \mathbf{x}, \mathbf{a}_{t}) p(\mathbf{x}| \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t-1}) 
    \label{eq:bayesian_filter:2}
\end{align}
Note that $p(\mathbf{x}| \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t}) = p(\mathbf{x}| \mathbf{z}_{1:t-1}, \mathbf{a}_{1:t-1})$, since we do not consider the state depending on future actions. 
%\todo[inline]{Dependence on actions is not super clear. Make this simplification more clear}
With equation \ref{eq:bayesian_filter:2}, we arrive at the formalization for object localization in the static case conditioned on the actions. 
\begin{equation}
    bel(\mathbf{x})_t = \eta p(\mathbf{z}_{t} | \mathbf{x}, \mathbf{a}_{t}) bel(\mathbf{x})_{t-1}
    \label{eq:bayesian_kalman}
\end{equation}
Note that the dependence of $\mathbf{x}$ on the actions is solemnly stemming from the measurement model $p(\mathbf{z}_{t} | \mathbf{x}, \mathbf{a}_{t})$. 
 
\subsubsection{Kalman Filter}
We assume that $\mathbf{x}$ and $\mathbf{z}_t$ are Gaussian distributed. The rotation $\mathbf{x}\in \mathbb{R}^4$ is parametrized as a quaternion. This gives a smooth representation over rotations in contrary to $SO(3)$. The measurements we obtain are actually 3D points from where the robot touched the object. In order to leverage the decoupling of rotation and translation we follow prior work of \cite{srivatsan2016estimating} and create a linear measurement model from the translation invariant measurements. We rearrange Equation \eqref{eq:trans_invariance} to
\begin{equation}
    \hat{\mathbf{a}_{ji}} - \mathbf{q} \odot \hat{\mathbf{b}_{ji}} \odot \mathbf{q}^{-1} = \mathbf{0} 
    \label{eq:quat_objective}
\end{equation}
by substituting with quaternions. Rewriting in matrix form as shown in \textit{Appendix} gives 
\begin{equation}
    \begin{bmatrix}
        0 & -(\mathbf{a}_{ji} - \mathbf{b}_{ij})^T \\
        (\mathbf{a}_{ji} + \mathbf{b}_{ji}) & (\mathbf{a}_j + \mathbf{a}_i + \mathbf{b}_j + \mathbf{b}_i)^{\times}
        \end{bmatrix}_{4x4} \hat{\mathbf{q}} = \mathbf{0} \quad .
        \label{eq:expected_measurement}
\end{equation}
We define this matrix as our measurement model and arrive at
\begin{equation}
    \mathbf{H}_t \mathbf{x} = \mathbf{z}_t
    \label{eq:measurement_model}
\end{equation}
The state that aligns the correspondences perfectly is given by the state $\mathbf{x}$, for which Equation \eqref{eq:measurement_model} becomes $0$. As in previous works we adopt the concept of pseudo-measurements. We set the true measurement always to $0$ and use equation \eqref{eq:measurement_model} as the expected measurement. With this we can formulate the simplified Kalman Equations as 

\begin{align}
    \mathbf{x}^*_{t|t} &= \mathbf{x}_{t-1|t-1} - \mathbf{K}_t \left( \mathbf{H}_t \mathbf{x}_{t-1|t-1} \right) \\
    \Sigma^{\mathbf{x}*}_{t|t} &= \left( \mathbf{I} - \mathbf{K}_t \mathbf{H}_t \right) \Sigma^{\mathbf{x}}_{t-1|t-1} \\
    \mathbf{K}_t &= \Sigma^\mathbf{x}_{t-1|t-1} \mathbf{H}^T \left( \mathbf{H}\Sigma^\mathbf{x}_{t-1|t-1} + \Sigma_t^{\mathbf{h}}\right) \quad . \label{eq:kalman_equations}
\end{align}

$\mathbf{x}_{t-1|t-1}$ is the mean of the state estimate at $t-1$, $\mathbf{K}_t$ is the kalman gain and $\Sigma^{\mathbf{x}}_{t-1|t-1}$ is the covariance matrix of the state at $t-1$. $\Sigma_t^{\mathbf{h}}$ is the measurement uncertainty at timestep $t$, which we define similar to \cite{srivatsan2016estimating}. To improve convergence speed we adopt a batch processing scheme similar to prior work. We construct $N_c$ matrices $\mathbf{H}_k$, where each matrix represents Equation \eqref{eq:trans_invariance} for one pair of measurements. We stack them in one matrix $\mathbf{G}_t$ to
\begin{equation}
    \mathbf{G}_t = \left[ \mathbf{H}_1, \ldots, \mathbf{H}_{N_c}\right] \in \mathbb{R}^{N_c \times 4} \quad .
\end{equation}
Therefore we are solving $N_c$ equations at the same time for the state that minimizes the alignment error. We replace matrix $\mathbf{H}_t$ in equation \eqref{eq:kalman_equations} with $\mathbf{G}_t$ to adopt the batch processing scheme. In order to ensure that the state represents a rotation, it has to be of unit length, i.e. a unit-quaternion. There are multiple strategies to enforce this. We however stick to previous works and normalize the state after the update to unit length with
\begin{equation}
    \mathbf{x}_{t|t} = \frac{\mathbf{x}^*_{t|t}}{||\mathbf{x}^{*}_{t|t}||_2} \quad \Sigma^{\mathbf{x}}_{t|t} = \frac{\Sigma^{\mathbf{x}*}_{t|t}}{||\mathbf{x}^{*}_{t|t}||_2^2}
\end{equation}
 
%===========================================================================

\subsection{Active Tactile Exploration}
To reduce the number of touches required to converge to the true position of the object, we need to make an informed decision on which action $a_t$ to perform next based on the current state estimate. As shown above we formulated a measurement model for the Kalman Filter, that depends on some action $\mathbf{a}_t$ that is chosen at timestep $t$. The set of all possible actions $\mathcal{A}(\mathbf{\mu}_t)$ depends on the current state-estimate $\mathbf{\mu}_t$. We want to select the action, $a_t \in \mathcal{A}(\mathbf{\mu}_t)$, that will lead to the measurement containing the most unseen information. To measure the information gain we use the KL divergence between $p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t})$ and $p(\mathbf{x} | \mathbf{z}_{1:t+1}, \mathbf{a}_{1:t+1})$. However, to get the true $p(\mathbf{x} | \mathbf{z}_{1:t+1}, \mathbf{a}_{1:t+1}$ we would have to perform the action $a_{t+1}$. Because of robot motion execution time this is very time consuming, therefore we approximate this distribution by using simulation. We choose a set of random actions from $\mathcal{A}(\mathbf{\mu}_t)$, obtain measurements $\hat{\mathbf{z}_{t+1}}$ from the simulation and then compute the resulting update of the distribution. This is repeated for $N_a$ samples. The chosen action $\mathbf{a}_{t+1}$ is then given by
\begin{align}
    &\mathbf{a}_{t+1} = \argmax_{\hat{\mathbf{a}}_{t+1} \in \mathcal{A}(\mathbf{\mu}_t)} KL(p(\mathbf{x} | \hat{\mathbf{z}}_{1:t+1},  \hat{\mathbf{a}}_{1:t+1}) || p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t})) \\
    &= \argmax_{\hat{\mathbf{a}}_{t+1} \in \mathcal{A}} \int_{x} p(\mathbf{x} | \hat{\mathbf{z}}_{1:t+1},  \hat{\mathbf{a}}_{1:t+1}) \log\frac{p(\mathbf{x} | \hat{\mathbf{z}}_{1:t+1},  \hat{\mathbf{a}}_{1:t+1})}{p(\mathbf{x} | \mathbf{z}_{1:t}, \mathbf{a}_{1:t})}dx \quad .
\end{align}
Since both distributions are gaussian, we can solve the above equation in closed form with
\begin{align}
    &\mathbf{a}_{t+1} = \argmax_{\hat{\mathbf{a}}_{t+1} \in \mathcal{A}} \frac{1}{2} \left[ \frac{|\Sigma_t|}{|\hat{\Sigma}_{t+1}|} -k + \right. \\
    &\left. (\hat{\mathbf{\mu}}_{t+1} - \mathbf{\mu}_{t})^T \Sigma_{t}^{-1} (\hat{\mathbf{\mu}}_{t+1} - \mathbf{\mu}_{t}) + Tr(\Sigma_{t}^{-1} \hat{\Sigma}_{t+1}) \vphantom{\frac{|\Sigma_t|}{|\hat{\Sigma}_{t+1}|}} \right]
\end{align}
% \todo[inline]{Define what k is in the equation above}

\subsubsection{Action Selection}
The relative entropy of the state belief at time $t$ is the Kullback-Leibler divergence of the posterior belief $bel(x_{t+1})$ and the prior belief $bel(x_t)$:
\begin{equation}
    IG = \int_{x} bel(x_{t+1})log\frac{bel(x_{t+1})}{bel(x_t)}dx \quad ,
\end{equation}
wherein, $IG$ measures the \textit{Information Gain} by performing a certain action. In the context of the \textit{best next touch} selection, we aim to find the action that \textit{maximises} the highest expected information gain. 
% \begin{itemize}
%     \item hypothetical measurement using future actions.
%     \item ray-mesh intersection for contact point estimation
% \end{itemize}

% \subsubsection{Termination Criteria}
% \begin{itemize}
%     \item Transformation epsilon between iterations
% \end{itemize}

\begin{algorithm}[h]
\SetAlgoLined
\KwResult{$\mathbf{q}$, $\mathbf{t}$, $\Sigma^{q}$}
\textbf{Input: }{$\mathbf{q_0}$, $\mathbf{t_0}$, $\epsilon_q$, $\epsilon_t$, $\mathbf{q_{gt}}$, $\mathbf{t_{gt}}$} \\ 
\textbf{Initialisation:} \\
Measurements point cloud $\mathcal{Z}$ = \{\} \\
Model point cloud $\mathcal{M}$ = $\mathcal{M}_{CAD}$ \\ 
Correspondences $\mathcal{C}$ = \{\} \\
Transform $\mathcal{M}$ to $q_0, t_0$ \\
Estimated Pose $\mathbf{\hat{q}}, \mathbf{t} \leftarrow \mathrm{MAX\_VALUE}$ \\
Initial Error $\Delta \mathbf{q} = abs(Eul(\mathbf{\hat{q}}) - Eul(\mathbf{q}))$, $\Delta \mathbf{t} = abs(Eul(\mathbf{\hat{q}}) - Eul(\mathbf{q}))$ \\ 
\While{$\Delta \mathbf{q} > \epsilon_q$ \&\& $\Delta \mathbf{t} > \epsilon_t$}{
    
    min, max $\leftarrow$ create\_bounding\_box($\mathcal{M}$) \;
    \eIf{size($\mathcal{Z}$) $\leq$ 2}{
        $\mathbf{a}$ = select\_random\_action($\mathbf{q}$, $\mathbf{t}$, $\mathcal{M}$) \\ 
    }
    {
        $a_i$, $\hat{z}_i$ = generate\_actions($\mathbf{q}$, $\mathbf{t}$, $\mathcal{M}$) \\
        Kullback–Leibler divergence $D_{KL}$ = \{\} \\
        \For{i=1 to size($a_i$)}{
            $\hat{\mathcal{S}}$ = $\mathcal{S} \cup \{ \}$ \;
            $\hat{\mathcal{C}}$ = est\_correspondences($\mathbf{q}$, $\mathbf{t}$, $\mathcal{M}$, $\hat{\mathcal{S}}$) \;
            $\hat{\mathbf{q}}$, $\hat{\Sigma}^q$, $\hat{\mathbf{t}}$ = tiq\_filter.update($\mathbf{q}$, $\Sigma^q$, $\hat{\mathcal{C}}$) \;
            KL.append(compute\_kl\_div($\hat{\mathbf{q}}$, $\hat{\Sigma}^q$, $\mathbf{q}$, $\Sigma^q$) \;
            
        $\mathbf{a}$ = $a_L$[argmax(KL)] \;
        }
     }
}   
\caption{Active tactile exploration for object localisation}
\end{algorithm}
